Analysing Diffusion-based Generative Approaches versus Discriminative Approaches for Speech Restoration

Diffusion-based generative models have had a high impact on the computer vision and speech processing communities these past years. Besides data generation tasks, they have also been employed for data restoration tasks like speech enhancement and dereverberation. While discriminative models have traditionally been argued to be more powerful e.g. for speech enhancement, generative diffusion approaches have recently been shown to narrow this performance gap considerably. In this paper, we systematically compare the performance of generative diffusion models and discriminative approaches on different speech restoration tasks. For this, we extend our prior contributions on diffusion-based speech enhancement in the complex time-frequency domain to the task of bandwith extension. We then compare it to a discriminatively trained neural network with the same network architecture on three restoration tasks, namely speech denoising, dereverberation and bandwidth extension. We observe that the generative approach performs globally better than its discriminative counterpart on all tasks, with the strongest benefit for non-additive distortion models, like in dereverberation and bandwidth extension. Code and audio examples can be found online at https://uhh.de/inf-sp-sgmsemultitask

==> biblio_waddress.tex <==
@STRING{ICASSP="IEEE Int. Conf. Acoustics, Speech, Signal Proc. (ICASSP)"}
@STRING{EUSIPCO={Proc. Euro. Signal Proc. Conf. (EUSIPCO)}}
@STRING{EUSIPJ={EURASIP Journal on Advances in Signal Proc.}}
@STRING{IWAENC={Int. Workshop on Acoustic Echo and Noise Control (IWAENC)}}
@STRING{TSAP={IEEE Trans. on Speech and Audio Proc.}}
@STRING{TASSP={IEEE Trans. on Acoustics, Speech and Signal Proc.}}
@STRING{TSP={IEEE Trans. on Signal Proc.}}
@STRING{SPM={IEEE Signal Proc. Magazine}}
@STRING{DAGA={DAGA -- Deutsche Arbeitsgemeinschaft f{\"u}r Akustik}}
@STRING{JASP={EURASIP J. Adv. Signal Proc.}}
@STRING{HSC={Int. Workshop on Hands-Free Speech Communication}}
@STRING{DEGA={Deutsche Jahrestagung f{\"u}r Akustik (DAGA)}}
@STRING{INTERSPEECH={Interspeech}}
@STRING{EUROSPEECH={ISCA Eurospeech}}
@STRING{ICSLP={Int. Conf. on Spoken Language Proc. (ICSLP)}}
@STRING{ESSV={Konferenz Elektronische Sprachsignalverarbeitung (ESSV)}}
@STRING{ELSEVIER={ELSEVIER Signal Proc.}}
@STRING{ELSESC={ELSEVIER Speech Communication}}
@STRING{JASA={J. Acoust. Soc. Am.}}
@STRING{SPL={IEEE Signal Proc. Letters}}
@STRING{TASLIEEE={IEEE Trans. Audio, Speech, Language Proc.}}
@STRING{TASL={IEEE/ACM Trans. Audio, Speech, Language Proc.}}
@STRING{TAP={IEEE Trans. on Antennas and Propagation}}
@STRING{ITG={ITG-Fachtagung Sprachkommunikation}}
@STRING{ASRU={IEEE Workshop Autom. Speech Recog. and Underst. (ASRU)}}
@STRING{ICML={Int. Conf. Machine Learning (ICML)}}
@STRING{ICLR={Int. Conf. Learning Repr. (ICLR)}}
@STRING{WASPAA={IEEE Workshop Applications Signal Proc. Audio, Acoustics (WASPAA)}}
@STRING{IWAENC={International Workshop on Acoustic Signal Enhancement}}
@STRING{NIPS={Neural Information Proc. Systems (NIPS)}}
@STRING{MLSP={IEEE Int. Workshop on Machine Learning for Signal Proc. (MLSP)}}

@book{bishop2006pattern,
author = {Bishop, Christopher},
title = {Pattern Recognition and Machine Learning},
year = {2006},
month = {January},
publisher = {Springer},
url = {https://www.microsoft.com/en-us/research/publication/pattern-recognition-machine-learning/},
}

@book{goodfellow2016deep,
  title={Deep learning},
  author={Goodfellow, Ian and Bengio, Yoshua and Courville, Aaron},
  year={2016},
  publisher={MIT press}
}

@book{Naylor2011,
title = {Speech Dereverberation},
author={Patrick A. Naylor and Nikolay D. Gaubitch},
year={2011},
volume = {59},
isbn = {978-1-84996-055-7},
publisher = {Noise Control Engineering Journal},
doi = {10.1007/978-1-84996-056-4},
publisher={Springer}
}

@ARTICLE{Nakatani2008a,  author={T. {Nakatani} and B. {Juang} and T. {Yoshioka} and K. {Kinoshita} and M. {Delcroix} and M. {Miyoshi}},  journal=TASLIEEE,   title={Speech Dereverberation Based on Maximum-Likelihood Estimation With Time-Varying {G}aussian Source Model},   year={2008},  volume={16},  number={8},  pages={1512-1527}}


@article{Jensen2016ESTOI,
author = {Jensen, Jesper and Taal, Cees},
year = {2016},
title = {An Algorithm for Predicting the Intelligibility of Speech Masked by Modulated Noise Maskers},
journal = TASL,
volume = 24,
number = 11,
pages = {2009-2022}
}


@ARTICLE{Yoshioka2012,  author={T. {Yoshioka} and T. {Nakatani}},  journal=TASLIEEE,   title={Generalization of Multi-Channel Linear Prediction Methods for Blind {MIMO} Impulse Response Shortening},   year={2012},  volume={20},  number={10},  pages={2707-2720},}


@ARTICLE{Vincent2006,
author={Vincent, E. and Gribonval, R. and Fevotte, C.},
journal=TASL, 
title={Performance measurement in blind audio source separation}, 
year={2006},
volume={14},
number={4},
pages={1462-1469},
doi={10.1109/TSA.2005.858005}}

@inproceedings{Caroselli2017,
  title={Adaptive Multichannel Dereverberation for Automatic Speech Recognition},
  author={J. Caroselli and I. Shafran and A. Narayanan and R. Rose},
  booktitle=INTERSPEECH,
  year={2017}
}

@article{Kuttruff2016,
    author={H. Kuttruff},
    title={Room acoustics},
    journal={CRC Press},
    year={2016}
    }
    
    
@article{Bradley2003,
title = {On the importance
of early reflections for speech in rooms},
journal = {The Journal of the Acoustical Society of America},
author={J. S. Bradley, H. Sato, and M. Picard},
year = {2003}
}

@ARTICLE{Yoshioka2012b,  author={Yoshioka, Takuya and Sehr, Armin and Delcroix, Marc and Kinoshita, Keisuke and Maas, Roland and Nakatani, Tomohiro and Kellermann, Walter},  journal=TSP,   title={Making Machines Understand Us in Reverberant Rooms: Robustness Against Reverberation for Automatic Speech Recognition},   year={2012},  volume={29},  number={6},  pages={114-126},  doi={10.1109/MSP.2012.2205029}}

@inproceedings{Kinoshita2017,
  title={Neural Network-Based Spectrum Estimation for Online {WPE} Dereverberation},
  author={K. Kinoshita and M. Delcroix and Haeyong Kwon and Takuma Mori and T. Nakatani},
  booktitle=INTERSPEECH,
  year={2017}
}

@article{Warzybok2003,
title = {Effects of spatial and temporal integration of a single early reflection on speech intelligibility},
author={A. Warzybok and J. Rennies and T. Brand, S. Doclo and B. Kollmeier},
journal = {The Journal of the Acoustical Society of America},
volume = {113},
number = {6},
pages = {2947-2952},
year = {2003},
doi = {10.1121/1.1577554}
}

@article{Markovich2009,  
author={Markovich, Shmulik and Gannot, Sharon and Cohen, Israel},  journal=TASL,   title={Multichannel Eigenspace Beamforming in a Reverberant Noisy Environment With Multiple Interfering Speech Signals},   year={2009},  volume={17},  number={6},  pages={1071-1086},  doi={10.1109/TASL.2009.2016395}}

@INPROCEEDINGS{Markovich2018,  author={Markovich-Golan, Shmulik and Gannot, Sharon},  booktitle={ICASSP 2015},   title={Performance analysis of the covariance subtraction method for relative transfer function estimation and comparison to the covariance whitening method},   year={2015},  volume={},  number={},  pages={544-548},  doi={10.1109/ICASSP.2015.7178028}}

@INPROCEEDINGS{Nakatani2008b,
  author={T. {Nakatani} and T. {Yoshioka} and K. {Kinoshita} and M. {Miyoshi} and B. {Juang}},
  booktitle={ICASSP 2008}, 
  title={Blind speech dereverberation with multi-channel linear prediction based on short time fourier transform representation}, 
  year={2008},
  volume={},
  number={},
  pages={85-88}}
  
@article{Wendt2014a,			  		  author={Wendt, Torben and  Van De Par, Steven and  Ewert, Stephan D.},					  journal={Journal of the Audio Engineering Society}, 					  title={A Computationally-efficient and perceptually-plausible algorithm for binaural room impulse response simulation}, 					  year={2014},					  volume={62},					  number={11},					  pages={748-766},					  doi={https://doi.org/10.17743/jaes.2014.0042},					  month={november},}						

@article{Wichern2019,
  author    = {Gordon Wichern and
               Joe Antognini and
               Michael Flynn and
               Licheng Richard Zhu and
               Emmett McQuinn and
               Dwight Crow and
               Ethan Manilow and
               Jonathan Le Roux},
  title     = {WHAM!: Extending Speech Separation to Noisy Environments},
  journal   = {CoRR},
  volume    = {abs/1907.01160},
  year      = {2019}
}

@inproceedings{Drude2018b,
  title={Integrating Neural Network Based Beamforming and Weighted Prediction Error Dereverberation},
  author={Lukas Drude and Christoph B{\"o}ddeker and Jahn Heymann and Reinhold Haeb-Umbach and Keisuke Kinoshita and Marc Delcroix and Tomohiro Nakatani},
  booktitle={INTERSPEECH},
  year={2018}
}

@article{Heymann2018,
  title={Frame-Online {DNN-WPE} Dereverberation},
  author={Jahn Heymann and Lukas Drude and Reinhold Haeb-Umbach and Keisuke Kinoshita and Tomohiro Nakatani},
  journal={IWAENC},
  year={2018},
  pages={466-470}
}

@INPROCEEDINGS{Heymann2019,
  title={Joint Optimization of Neural Network-based {WPE} Dereverberation and Acoustic Model for Robust Online {ASR}},
  author={Jahn Heymann and Lukas Drude and Reinhold Haeb-Umbach and Keisuke Kinoshita and Tomohiro Nakatani},
  booktitle=ICASSP,
  year={2019}
}

@INPROCEEDINGS{Nakatani2020,  author={T. {Nakatani} and R. {Takahashi} and T. {Ochiai} and K. {Kinoshita} and R. {Ikeshita} and M. {Delcroix} and S. {Araki}},  booktitle={ICASSP},   title={DNN-supported Mask-based Convolutional Beamforming for Simultaneous Denoising, Dereverberation, and Source Separation},   year={2020},  volume={},  number={},  pages={6399-6403},  doi={10.1109/ICASSP40776.2020.9053343}}

@phdthesis{Carbajal2020,
  title={Apprentissage profond bout-en-bout pour le rehaussement de la parole},
  author={Carbajal, Guillaume},
  year={2020},
  school={Universit{\'e} de Lorraine}
}

@article{Duong2013,
	title = {Spatial location priors for {Gaussian} model based reverberant audio source separation},
	volume = {2013},
	issn = {1687-6180},
	number = {1},
	urldate = {2020-10-06},
	journal = EUSIPJ,
	author = {Duong, Ngoc Q K and Vincent, Emmanuel and Gribonval, Rémi},
	month = dec,
	year = {2013},
	pages = {149}
}

@INPROCEEDINGS{Ito2018,  author={N. {Ito} and C. {Schymura} and S. {Araki} and T. {Nakatani}},  booktitle=EUSIPCO,   title={Noisy cGMM: Complex Gaussian Mixture Model with Non-Sparse Noise Model for Joint Source Separation and Denoising},   year={2018},  volume={},  number={},  pages={1662-1666},  doi={10.23919/EUSIPCO.2018.8553410}}

@ARTICLE{Nikunen2014,  author={J. {Nikunen} and T. {Virtanen}},  journal=TASL,   title={Direction of Arrival Based Spatial Covariance Model for Blind Sound Source Separation},   year={2014},  volume={22},  number={3},  pages={727-739}}

@ARTICLE{Pang2019,  author={C. {Pang} and H. {Liu} and X. {Li}},  journal={IEEE Access},   title={Multitask Learning of Time-Frequency CNN for Sound Source Localization},   year={2019},  volume={7},  number={},  pages={40725-40737}}

@INPROCEEDINGS{Adavanne2018,  author={S. {Adavanne} and A. {Politis} and T. {Virtanen}},  booktitle={EUSIPCO},   title={Direction of Arrival Estimation for Multiple Sound Sources Using Convolutional Recurrent Neural Network},   year={2018},  volume={},  number={},  pages={1462-1466}}

@INPROCEEDINGS{Boedekker2020,  author={C. {Boeddeker} and T. {Nakatani} and K. {Kinoshita} and R. {Haeb-Umbach}},  booktitle=ICASSP,   title={Jointly Optimal Dereverberation and Beamforming},   year={2020},  volume={},  number={},  pages={216-220},  doi={10.1109/ICASSP40776.2020.9054393}}

@inproceedings{Xue2020,
  author={Wei Xue and Ying Tong and Chao Zhang and Guohong Ding and Xiaodong He and Bowen Zhou},
  title={{Sound Event Localization and Detection Based on Multiple DOA Beamforming and Multi-Task Learning}},
  year=2020,
  booktitle=INTERSPEECH,
  pages={5091--5095},
  doi={10.21437/Interspeech.2020-2759},
  url={http://dx.doi.org/10.21437/Interspeech.2020-2759}
}

@ARTICLE{Nakatani2019,  author={T. {Nakatani} and K. {Kinoshita}},  journal=SPL,   title={A Unified Convolutional Beamformer for Simultaneous Denoising and Dereverberation},   year={2019},  volume={26},  number={6},  pages={903-907},  doi={10.1109/LSP.2019.2911179}}

@inproceedings{Nakatani2019b,
  title={Simultaneous Denoising and Dereverberation for Low-Latency Applications Using Frame-by-Frame Online Unified Convolutional Beamformer},
  author={T. Nakatani and K. Kinoshita},
  booktitle=INTERSPEECH,
  year={2019}
}

@article{Ni2021,
  title={WPD++: An Improved Neural Beamformer for Simultaneous Speech Separation and Dereverberation},
  author={Zhaoheng Ni and Yanchen Xu and Meng Yu and Bo Wu and S. Zhang and Dong Yu and Michael I. Mandel},
  journal={2021 IEEE Spoken Language Technology Workshop (SLT)},
  year={2021},
  pages={817-824}
}

@INPROCEEDINGS{Revach2021,  author={Revach, Guy and Shlezinger, Nir and van Sloun, Ruud J. G. and Eldar, Yonina C.},  journal=ICASSP,   title={Kalmannet: Data-Driven Kalman Filtering},   year={2021},  volume={},  number={},  pages={3905-3909},  doi={10.1109/ICASSP39728.2021.9413750}}

@ARTICLE{Braun2016,  author={Braun, Sebastian and Habets, Emanuël A. P.},  journal=SPL,   title={Online Dereverberation for Dynamic Scenarios Using a {K}alman Filter With an Autoregressive Model},   year={2016},  volume={23},  number={12},  pages={1741-1745},  doi={10.1109/LSP.2016.2616888}}

@ARTICLE{Braun2018,  author={Braun, Sebastian and Habets, Emanuël A. P.},  journal=TASL,   title={Linear Prediction-Based Online Dereverberation and Noise Reduction Using Alternating Kalman Filters},   year={2018},  volume={26},  number={6},  pages={1119-1129},  doi={10.1109/TASLP.2018.2811247}}

@INPROCEEDINGS{Braun2020,  author={Hashemgeloogerdi, Sahar and Braun, Sebastian},  journal=ICASSP,   title={Joint Beamforming and Reverberation Cancellation Using a Constrained {K}alman Filter With Multichannel Linear Prediction},   year={2020},  volume={},  number={},  pages={481-485},  doi={10.1109/ICASSP40776.2020.9053785}}

@ARTICLE{Schwartz2015,  author={Schwartz, Boaz and Gannot, Sharon and Habets, Emanuël A. P.},  journal=TASL,   title={Online Speech Dereverberation Using {K}alman Filter and {EM} Algorithm},   year={2015},  volume={23},  number={2},  pages={394-406},  doi={10.1109/TASLP.2014.2372342}}

@misc{Maciejewski2020,
      title={WHAMR!: Noisy and Reverberant Single-Channel Speech Separation}, 
      author={Matthew Maciejewski and Gordon Wichern and Emmett McQuinn and Jonathan Le Roux},
      year={2020},
      eprint={1910.10279},
      archivePrefix={arXiv},
      primaryClass={cs.SD}
}

@ARTICLE{Yoshioka2011,  author={Yoshioka, Takuya and Nakatani, Tomohiro and Miyoshi, Masato and Okuno, Hiroshi G.},  journal=TASLIEEE,   title={Blind Separation and Dereverberation of Speech Mixtures by Joint Optimization},   year={2011},  volume={19},  number={1},  pages={69-84},  doi={10.1109/TASL.2010.2045183}}

@INPROCEEDINGS{Baby2021,  author={Baby, Deepak and Bourlard, Hervé},  booktitle=ICASSP,   title={Speech Dereverberation Using Variational Autoencoders},   year={2021},  volume={},  number={},  pages={5784-5788},  doi={10.1109/ICASSP39728.2021.9414736}}

@ARTICLE{Carbajal2020b,  author={Carbajal, Guillaume and Serizel, Romain and Vincent, Emmanuel and Humbert, Eric},  journal=TASL,   title={Joint {NN}-Supported Multichannel Reduction of Acoustic Echo, Reverberation and Noise},   year={2020},  volume={28},  number={},  pages={2158-2173},  doi={10.1109/TASLP.2020.3008974}}

@article{Cauchi2015,
  title={Combination of {MVDR} beamforming and single-channel spectral processing for enhancing noisy and reverberant speech},
  author={Benjamin Cauchi and I. Kodrasi and R. Rehr and Stephan Gerlach and Ante Jukic and Timo Gerkmann and S. Doclo and Stefan Goetze},
  journal=EUSIPJ,
  year={2015},
  volume={2015},
  pages={1-12}
}

@ARTICLE{Jukic2015,  author={Jukić, Ante and van Waterschoot, Toon and Gerkmann, Timo and Doclo, Simon},  journal=TASL,   title={Multi-Channel Linear Prediction-Based Speech Dereverberation With Sparse Priors},   year={2015},  volume={23},  number={9},  pages={1509-1520},  doi={10.1109/TASLP.2015.2438549}}

@misc{Choi2020,
      title={Phase-aware Single-stage Speech Denoising and Dereverberation with U-Net}, 
      author={Hyeong-Seok Choi and Hoon Heo and Jie Hwan Lee and Kyogu Lee},
      year={2020},
      eprint={2006.00687},
      archivePrefix={arXiv},
      primaryClass={eess.AS}
}

@INPROCEEDINGS{Cohen2017,  author={Cohen, Alejandro and Stemmer, Georg and Ingalsuo, Seppo and Markovich-Golan, Shmulik},  journal=ICASSP,   title={Combined Weighted Prediction Error and Minimum Variance Distortionless Response for dereverberation},   year={2017},  volume={},  number={},  pages={446-450},  doi={10.1109/ICASSP.2017.7952195}}

@inproceedings{Ernst2019,
      title={Speech Dereverberation Using Fully Convolutional Networks}, 
      author={Ori Ernst and Shlomo E. Chazan and Sharon Gannot and Jacob Goldberger},
      year={2019},
      booktitle=EUSIPCO,
      month=sep,
      address={A Coru{\~{n}}a, Spain}
}

@INPROCEEDINGS{Kinoshita2006,  author={Kinoshita, K. and Nakatani, T. and Miyoshi, M.},  journal=ICASSP,   title={Spectral Subtraction Steered by Multi-Step Forward Linear Prediction For Single Channel Speech Dereverberation},   year={2006},  volume={1},  number={},  pages={I-I},  doi={10.1109/ICASSP.2006.1660146}}

@inproceedings{Luo2018,
  title={Real-time Single-channel Dereverberation and Separation with Time-domain Audio Separation Network},
  author={Yi Luo and N. Mesgarani},
  booktitle=Interspeech,
  year={2018}
}

@ARTICLE{Han2017,  author={Han, Kun and Wang, Yuxuan and Wang, DeLiang and Woods, William S. and Merks, Ivo and Zhang, Tao},  journal=TASL,   title={Learning Spectral Mapping for Speech Dereverberation and Denoising},   year={2015},  volume={23},  number={6},  pages={982-992},  doi={10.1109/TASLP.2015.2416653}}

@INPROCEEDINGS{Mosayyebpour2018,  author={Mosayyebpour, Saeed and Nesta, Francesco},  booktitle=EUSIPCO,   title={Neural-Network Supervised Maximum Likelihood-based on-line Dereverberation},   year={2018},  volume={},  number={},  pages={1552-1556},  doi={10.23919/EUSIPCO.2018.8553143}}

@ARTICLE{Tan2020,  author={Tan, Ke and Xu, Yong and Zhang, Shi-Xiong and Yu, Meng and Yu, Dong},  journal={IEEE Journal of Selected Topics in Signal Processing},   title={Audio-Visual Speech Separation and Dereverberation With a Two-Stage Multimodal Network},   year={2020},  volume={14},  number={3},  pages={542-553},  doi={10.1109/JSTSP.2020.2987209}}

@ARTICLE{Schwarz2015,  author={Schwarz, Andreas and Kellermann, Walter},  journal=TASL,   title={Coherent-to-Diffuse Power Ratio Estimation for Dereverberation},   year={2015},  volume={23},  number={6},  pages={1006-1018},  doi={10.1109/TASLP.2015.2418571}}

@ARTICLE{Wung2020,  author={Wung, Jason and Jukić, Ante and Malik, Sarmad and Souden, Mehrez and Pichevar, Ramin and Atkins, Joshua and Naik, Devang and Acero, Alex},  journal=TSP,   title={Robust Multichannel Linear Prediction for Online Speech Dereverberation Using Weighted {H}ouseholder Least Squares Lattice Adaptive Filter},   year={2020},  volume={68},  number={},  pages={3559-3574},  doi={10.1109/TSP.2020.2997201}}

@INPROCEEDINGS{Kuklasinski2015,  author={Kuklasiński, Adam and Doclo, Simon and Gerkmann, Timo and Holdt Jensen, Søren and Jensen, Jesper},  booktitle=ICASSP,   title={Multi-channel {PSD} estimators for speech dereverberation - A theoretical and experimental comparison},   year={2015}, pages={91-95}}

@INPROCEEDINGS{Wang2021,  author={Wang, Zhong-Qiu and Wang, DeLiang},  journal=ICASSP,   title={Multi-Microphone Complex Spectral Mapping for Speech Dereverberation},   year={2020},  volume={},  number={},  pages={486-490},  doi={10.1109/ICASSP40776.2020.9053610}}

@INPROCEEDINGS{Zhang2021,
      title={End-to-End Dereverberation, Beamforming, and Speech Recognition with Improved Numerical Stability and Advanced Frontend}, 
      author={Wangyou Zhang and Christoph Boeddeker and Shinji Watanabe and Tomohiro Nakatani and Marc Delcroix and Keisuke Kinoshita and Tsubasa Ochiai and Naoyuki Kamo and Reinhold Haeb-Umbach and Yanmin Qian},
      year={2021},
      booktitle=ICASSP
}

@misc{Zhang2020,
      title={End-to-End Far-Field Speech Recognition with Unified Dereverberation and Beamforming}, 
      author={Wangyou Zhang and Aswin Shanmugam Subramanian and Xuankai Chang and Shinji Watanabe and Yanmin Qian},
      year={2020},
      eprint={2005.10479},
      archivePrefix={arXiv},
      primaryClass={eess.AS}
}

@phdthesis{Habets2007,
author = {Habets, Emanuël},
year = {2007},
title = {Single- and Multi-Microphone Speech Dereverberation Using Spectral Enhancement},
journal = {Journal of The ACM - JACM}
}

@article{Hu2014,
author = {Hu, Yi and Kokkinakis, Kostas},
year = {2014},
month = {01},
pages = {EL22-8},
title = {Effects of early and late reflections on intelligibility of reverberated speech by cochlear implant listeners},
volume = {135},
journal = {The Journal of the Acoustical Society of America},
doi = {10.1121/1.4834455}
}

@INPROCEEDINGS{Kagami2018,  author={Kagami, Hideaki and Kameoka, Hirokazu and Yukawa, Masahiro},  booktitle=ICASSP,   title={Joint Separation and Dereverberation of Reverberant Mixtures with Determined Multichannel Non-Negative Matrix Factorization},   year={2018},  volume={},  number={},  pages={31-35},  doi={10.1109/ICASSP.2018.8462080}}

@ARTICLE{Ochiai2017,  author={Ochiai, Tsubasa and Watanabe, Shinji and Hori, Takaaki and Hershey, John R. and Xiao, Xiong},  journal={IEEE Journal of Selected Topics in Signal Proc.},   title={Unified Architecture for Multichannel End-to-End Speech Recognition With Neural Beamforming},   year={2017},  volume={11},  number={8},  pages={1274-1288},  doi={10.1109/JSTSP.2017.2764276}}

@article{Chang2019,
  title={MIMO-Speech: End-to-End Multi-Channel Multi-Speaker Speech Recognition},
  author={Xuankai Chang and Wangyou Zhang and Y. Qian and Jonathan Le Roux and Shinji Watanabe},
  journal={2019 IEEE Automatic Speech Recognition and Understanding Workshop (ASRU)},
  year={2019},
  pages={237-244}
}

@INPROCEEDINGS{Williamson2017,  author={Williamson, Donald S. and Wang, DeLiang},  booktitle=ICASSP,   title={Speech dereverberation and denoising using complex ratio masks},   year={2017},  volume={},  number={},  pages={5590-5594},  doi={10.1109/ICASSP.2017.7953226}}

@ARTICLE{Williamson2017j,  author={Williamson, Donald S. and Wang, DeLiang},  journal=TASL,   title={Time-Frequency Masking in the Complex Domain for Speech Dereverberation and Denoising},   year={2017},  volume={25},  number={7},  pages={1492-1501},  doi={10.1109/TASLP.2017.2696307}}

@article{Valin2018,
  title={A Hybrid DSP/Deep Learning Approach to Real-Time Full-Band Speech Enhancement},
  author={Jean-Marc Valin},
  journal={2018 IEEE 20th International Workshop on Multimedia Signal Processing (MMSP)},
  year={2018},
  pages={1-5}
}

@inproceedings{Li2021,
  author={Andong Li and Wenzhe Liu and Xiaoxue Luo and Guochen Yu and Chengshi Zheng and Xiaodong Li},
  title={{A Simultaneous Denoising and Dereverberation Framework with Target Decoupling}},
  year=2021,
  booktitle={Proc. Interspeech 2021},
  pages={2801--2805},
  doi={10.21437/Interspeech.2021-1137}
}

@INPROCEEDINGS{Kodrasi2014,  author={Kodrasi, Ina and Gerkmann, Timo and Doclo, Simon},  booktitle=ICASSP,   title={Frequency-domain single-channel inverse filtering for speech dereverberation: Theory and practice},   year={2014},  
month=may,
address = {Florence, Italy}}


@article{Allen1977,
author = {Allen,J. B.  and Berkley,D. A.  and Blauert,J. },
title = {Multimicrophone signal‐processing technique to remove room reverberation from speech signals},
journal = {The Journal of the Acoustical Society of America},
volume = {62},
number = {4},
pages = {912-915},
year = {1977}
}
@INPROCEEDINGS{Gerkmann2011,  author={Gerkmann, Timo},  booktitle=EUSIPCO,   title={Cepstral weighting for speech dereverberation without musical noise},   year={2011},
month=sep,
address={Barcelona, Spain}}

@misc{Tesch2022J,
  author = {Tesch, Kristina and Gerkmann, Timo},
  title = {Insights into Deep Non-linear Filters for Improved Multi-channel Speech Enhancement},
  journal = {arXiv},
  year = {2022}
}


@article{Andreev2022Hifi++,
  author = {Andreev, Pavel and Alanov, Aibek and Ivanov, Oleg and Vetrov, Dmitry},
  title = {HiFi++: a Unified Framework for Bandwidth Extension and Speech Enhancement},
  year = {2022},
  journal = {arXiv}
}

@inproceedings{Lin2021TwoStageBWE,
  title={A Two-Stage Approach to Speech Bandwidth Extension},
  author={Ju Lin and Yun Wang and Kaustubh Kalgaonkar and Gil Keren and Didi Zhang and Christian Fuegen},
  booktitle=Interspeech,
  year={2021},
  month=sep,
  adress={Brno, Czech Republic}
}

@inproceedings{Kuleshov2017AudioSuperResolution,
  author = {Kuleshov, Volodymyr and Enam, S. Zayd and Ermon, Stefano},
  title = {Audio Super Resolution using Neural Networks},
  year = {2017},
  booktitle=ICLR
 }
 
@inproceedings{Birnbaum2017TFiLM,
  author = {Birnbaum, Sawyer and Kuleshov, Volodymyr and Enam, Zayd and Koh, Pang Wei and Ermon, Stefano},
  title = {Temporal FiLM: Capturing Long-Range Sequence Dependencies with Feature-Wise Modulations},
  year = {2019},
  booktitle=NIPS,
  month = dec,
  address = {Vancouver, Canada}
  }

@inproceedings{Wang2020TimeFrequencyLF,
  title={Time-Frequency Loss for CNN Based Speech Super-Resolution},
  author={Heming Wang and Deliang Wang},
  booktitle=ICASSP,
  year={2020},
}

@inproceedings{Li2015DNNbasedSB,
  title={DNN-based speech bandwidth expansion and its application to adding high-frequency missing features for automatic speech recognition of narrowband speech},
  author={Kehuang Li and Zhen Huang and Yong Xu and Chin-Hui Lee},
  booktitle=INTERSPEECH,
  year={2015}
}

@article{Liu2021VoiceFixer,
  author = {Liu, Haohe and Kong, Qiuqiang and Tian, Qiao and Zhao, Yan and Wang, DeLiang and Huang, Chuanzeng and Wang, Yuxuan},
  title = {VoiceFixer: Toward General Speech Restoration with Neural Vocoder},
  year = {2021},
  journal={arXiv}
}

@inproceedings{Welker2022SGMSE,
      title={Speech Enhancement with Score-Based Generative Models in the Complex {STFT} Domain}, 
      author={Simon Welker and Julius Richter and Timo Gerkmann},
      year={2022},
      booktitle=Interspeech,
      month=sep,
      address={Incheon, South Korea}
}

@article{Richter2022SGMSE++,
      title={Speech Enhancement and Dereverberation with Diffusion-based Generative Models}, 
      author={Julius Richter and Simon Welker and Jean-Marie Lemercier and Bunlong Lay and Timo Gerkmann},
      year={2022},
      journal={arXiv}
}

@book{hendriks2013dft,
  title = {{DFT}-domain based single-microphone noise reduction for speech enhancement: A survey of the state-of-the-art},
  author = {Hendriks, Richard C. and Gerkmann, Timo and Jensen, Jesper},
  year = {2013},
  publisher = {Morgan \& Claypool}
}

@book{Godsill1998DigitalAR,
  title={Digital audio restoration},
  author={Simon J. Godsill and Peter J. W. Rayner and Olivier Capp{\'e}},
  publisher={Springer},
  year={1998}
}

@incollection{gerkmann2018book_chapter,
    author  = {Gerkmann, Timo and Vincent, Emmanuel},
    editor  = {Vincent, Emmanuel},
    year    = {2018},
    title   = {Spectral Masking and Filtering},
    booktitle   = {Audio Source Separation and Speech Enhancement},
    publisher   = {John Wiley \& Sons},
}

@article{wang2018supervised,
  title={Supervised speech separation based on deep learning: An overview},
  author={Wang, DeLiang and Chen, Jitong},
  journal=TASLIEEE,
  year={2018},
  volume={26},
  number={10},
  pages={1702-1726}
  }

@inproceedings{Rezende2015Normalizing,
  author = {Rezende, Danilo Jimenez and Mohamed, Shakir},
  title = {Variational Inference with Normalizing Flows},
  year = {2015},
  booktitle=ICML
}

@article{Kobyzev2021NFOverview,
	year = 2021,
	month = {nov},
	volume = {43},
	number = {11},
	pages = {3964--3979},
	author = {Ivan Kobyzev and Simon J.D. Prince and Marcus A. Brubaker},
	title = {Normalizing Flows: An Introduction and Review of Current Methods},
	journal = {{IEEE} Transactions on Pattern Analysis and Machine Intelligence}
}

@inproceedings{Song2020Improved,
  author = {Song, Yang and Ermon, Stefano},
  title = {Improved Techniques for Training Score-Based Generative Models},
  year = {2020},
  booktitle=NIPS
}

@inproceedings{Kingma2021VDM,
  author = {Kingma, Diederik P. and Salimans, Tim and Poole, Ben and Ho, Jonathan},
  title = {Variational Diffusion Models},
  year = {2021},
booktitle=NIPS,
}

@article{vincent2011connection,
  author={Vincent, Pascal},
  journal={Neural Computation}, 
  title={A Connection Between Score Matching and Denoising Autoencoders}, 
  year={2011},
  volume={23},
  number={7},
  pages={1661-1674},
}

@article{hyvarinen2005estimation,
  title={Estimation of non-normalized statistical models by score matching.},
  author={Hyv{\"a}rinen, Aapo and Dayan, Peter},
  journal={Journal of Machine Learning Research},
  year={2005},
  volume=6,
  pages={695–709}
}

@article{richter2020speech,
  title={Speech Enhancement with Stochastic Temporal Convolutional Networks.},
  author={Richter, Julius and Carbajal, Guillaume and Gerkmann, Timo},
  journal=INTERSPEECH,
  year={2020}
}

@article{carbajal2021disentanglement,
  title={Disentanglement Learning for Variational Autoencoders Applied to Audio-Visual Speech Enhancement},
  author={Carbajal, Guillaume and Richter, Julius and Gerkmann, Timo},
  journal=WASPAA,
  pages={126--130},
  year={2021},
}

@inproceedings{fang2021variational,
  title={Variational autoencoder for speech enhancement with a noise-aware encoder},
  author={Fang, Huajian and Carbajal, Guillaume and Wermter, Stefan and Gerkmann, Timo},
  journal=ICASSP,
  year={2021},
  month=jun,
  address={Toronto, Canada}
}

@article{kingma2014auto,
  author={Diederik P. Kingma and Max Welling},
  title={Auto-encoding variational {Bayes}},
  journal=ICLR,
  year={2014},
}

@article{goodfellow2014generative,
  title={Generative adversarial networks},
  author={Goodfellow, Ian and Pouget-Abadie, Jean and Mirza, Mehdi and Xu, Bing and Warde-Farley, David and Ozair, Sherjil and Courville, Aaron and Bengio, Yoshua},
  booktitle=NIPS,
  volume={27},
  year={2014}
}

@inproceedings{sohl2015deep,
  title={Deep unsupervised learning using nonequilibrium thermodynamics},
  author={Sohl-Dickstein, Jascha and Weiss, Eric and Maheswaranathan, Niru and Ganguli, Surya},
  booktitle=ICML,
  year={2015},
address = {Lille, France},
month = apr
}

@article{koizumi2022specgrad,
  title={{SpecGrad}: Diffusion Probabilistic Model based Neural Vocoder with Adaptive Noise Spectral Shaping},
  author={Koizumi, Yuma and Zen, Heiga and Yatabe, Kohei and Chen, Nanxin and Bacchiani, Michiel},
  journal=INTERSPEECH,
  year={2022}
}

@inproceedings{song2019generative,
  title={Generative modeling by estimating gradients of the data distribution},
  author={Song, Yang and Ermon, Stefano},
  booktitle=NIPS,
  year={2019},
  month = dec,
  address = {Vancouver, Canada}
}

@inproceedings{ho2020denoising,
  title={Denoising diffusion probabilistic models},
  author={Ho, Jonathan and Jain, Ajay and Abbeel, Pieter},
  booktitle=NIPS,
  year={2020},
  month=dec,
  address = {Online}
}

@article{leglaive2018variance,
  title={A variance modeling framework based on variational autoencoders for speech enhancement},
  author={Leglaive, Simon and Girin, Laurent and Horaud, Radu},
  journal=MLSP,
  pages={1--6},
  year={2018},
}

@inproceedings{lu2021study,
  title={A Study on Speech Enhancement Based on Diffusion Probabilistic Model},
  author={Lu, Yen-Ju and Tsao, Yu and Watanabe, Shinji},
  booktitle={Asia-Pacific Signal and Information Processing Association (APSIPA)},
  year={2021},
  month=dec,
  address = {Tokyo, Japan}
}

@inproceedings{lu2022conditional,
  title={Conditional diffusion probabilistic model for speech enhancement},
  author={Lu, Yen-Ju and Wang, Zhong-Qiu and Watanabe, Shinji and Richard, Alexander and Yu, Cheng and Tsao, Yu},
  booktitle=ICASSP,
  year={2022},
  month=jun,
  address={Singapore, Singapore}
}

@article{bando2020adaptive,
  title={Adaptive Neural Speech Enhancement with a Denoising Variational Autoencoder.},
  author={Bando, Yoshiaki and Sekiguchi, Kouhei and Yoshii, Kazuyoshi},
  journal=INTERSPEECH,
  year={2020}
}

@inproceedings{dhariwal2021diffusion,
  title={Diffusion models beat {GANs} on image synthesis},
  author={Dhariwal, Prafulla and Nichol, Alexander},
  journal=NIPS,
  volume={34},
  year={2021}
}

@article{kong2021diffwave,
  title={{DiffWave}: A Versatile Diffusion Model for Audio Synthesis},
  author={Zhifeng Kong and Wei Ping and Jiaji Huang and Kexin Zhao and Bryan Catanzaro},
  journal=ICLR,
  year={2021}
}

@article{chen2021wavegrad,
  title={{WaveGrad}: Estimating Gradients for Waveform Generation},
  author={Nanxin Chen and Yu Zhang and Heiga Zen and Ron J Weiss and Mohammad Norouzi and William Chan},
  journal=ICLR,
  year={2021}
}

@inproceedings{song2021sde,
  title={Score-Based Generative Modeling through Stochastic Differential Equations},
  author={Yang Song and Jascha Sohl-Dickstein and Diederik P Kingma and Abhishek Kumar and Stefano Ermon and Ben Poole},
  booktitle=ICLR,
  year={2021},
  month = may,
  address = {Online}
}

@article{serra2022universal,
  title={Universal Speech Enhancement with Score-based Diffusion},
  author={Serr{\`a}, Joan and Pascual, Santiago and Pons, Jordi and Araz, R Oguz and Scaini, Davide},
  journal={arXiv},
  year={2022}
}

@article{anderson1982reverse,
  title={Reverse-time diffusion equation models},
  author={Anderson, Brian DO},
  journal={Stochastic Processes and their Applications},
  year={1982},
  volume=12,
  number=3,
  pages={313-326},
  publisher={Elsevier}
}

@ARTICLE{Han2015,  author={Han, Kun and Wang, Yuxuan and Wang, DeLiang and Woods, William S. and Merks, Ivo and Zhang, Tao},  journal=TASL,   title={Learning Spectral Mapping for Speech Dereverberation and Denoising},   year={2015}}

@article{Li2022,
title = {Glance and gaze: A collaborative learning framework for single-channel speech enhancement},
journal = {Applied Acoustics},
year = {2022},
author = {Andong Li and Chengshi Zheng and Lu Zhang and Xiaodong Li}}

@ARTICLE{Noll1993,  author={Noll, P.},  journal={IEEE Communications Magazine},   title={Wideband speech and audio coding},   year={1993},  volume={31},  number={11},  pages={34-44},  doi={10.1109/35.256878}}

@inbook{Chiu2004,
    title={Speech Coding Algorithms},
    author={Wai C. Chiu},
    publisher={Wiley-Interscience},
    year=2004
}

@INPROCEEDINGS{Brauer2016,  author={Brauer, Christoph and Gerkmann, Timo and Lorenz, Dirk},  booktitle=ICASSP,   title={Sparse reconstruction of quantized speech signals},   year={2016}}

@inproceedings{Nguyen2022Tunet,
	year = 2022,
	author = {Viet-Anh Nguyen and Anh H. T. Nguyen and Andy W. H. Khong},
	title = {{TUN}et: A Block-Online Bandwidth Extension Model Based On Transformers And Self-Supervised Pretraining},
	booktitle = ICASSP,
 month=jun,
 address={Singapore, Singapore}
}

@article{Zaviska2021DeclippingSurvey,
	year = 2021,
	month = {jan},
	volume = {15},
	number = {1},
	pages = {5--24},
	author = {Pavel Zaviska and Pavel Rajmic and Alexey Ozerov and Lucas Rencker},
	title = {A Survey and an Extensive Evaluation of Popular Audio Declipping Methods},
	journal = {{IEEE} Journal of Selected Topics in Signal Processing}
}

@article{Deng2019ExploitingTP,
  title={Exploiting time-frequency patterns with LSTM-RNNs for low-bitrate audio restoration},
  author={Jun Deng and Bj{\"o}rn Schuller and Florian Eyben and Dagmar M. Schuller and Zixing Zhang and Holly Francois and Eunmi L. Oh},
  journal={Neural Computing and Applications},
  year={2019},
  volume={32},
  pages={1095-1107}
}

@article{Eskimez2019AdversarialTF,
  title={Adversarial Training for Speech Super-Resolution},
  author={Sefik Emre Eskimez and Kazuhito Koishida and Zhiyao Duan},
  journal={IEEE Journal of Selected Topics in Signal Processing},
  year={2019},
  volume={13},
  pages={347-358}
}

@article{Dietz2002SpectralBR,
  title={Spectral Band Replication, a Novel Approach in Audio Coding},
  author={Martin Dietz and Lars Gustaf Liljeryd and Kristofer Kj{\"o}rling and Oliver Kunz},
  journal={Journal of The Audio Engineering Society},
  year={2002}
}

@incollection{Disch2017,
author = {S Disch and T Bäckström},
year = {2017},
title = {Bandwidth Extension},
booktitle = {Speech Coding with Code-Excited Linear Prediction},
publisher=Springer
}

@article{Liu2010AHB,
  title={A harmonic bandwidth extension based on Gaussian mixture model},
  author={Xin Liu and Chang-chun Bao and Mao-shen Jia and Yong-tao Sha},
  journal=ICASSP,
  year={2010},
}

@book{Oksendal2000SDE,
author = {Øksendal, Bernt},
year = {2000},
pages = {},
title = {Stochastic Differential Equations: An Introduction with Applications},
volume = {82},
isbn = {978-3-540-60243-9},
publisher = {Journal of the American Statistical Association},
doi = {10.1007/978-3-662-03185-8}
}

@misc{datasetWSJ0,
  title = {{{CSR-I}} ({{WSJ0}}) {{Complete}}},
  author = {Garofolo, John S. and Graff, David and Paul, Doug and Pallett, David},
  year=2007,
  month=may,
  publisher = {{Linguistic Data Consortium}},
  url = {https://catalog.ldc.upenn.edu/LDC93S6A},
  urldate = {2021-11-19}
}

@inproceedings{valentini2016investigating,
  title={Investigating {RNN}-based speech enhancement methods for noise-robust Text-to-Speech},
  author={Valentini-Botinhao, Cassia and Wang, Xin and Takaki, Shinji and Yamagishi, Junichi},
  booktitle = {Speech Synthesis Workshop (SSW)},
  year={2016},
  month = sep,
  address = {Sunnyvale, USA}
}

@article{barker2015third,
  title={The third ‘{CHiME}’ speech separation and recognition challenge: Dataset, task and baselines},
  author={Barker, Jon and Marxer, Ricard and Vincent, Emmanuel and Watanabe, Shinji},
  journal={IEEE Workshop on Automatic Speech Recognition and Understanding (ASRU)},
  year={2015},
  month = dec,
  address = {Scottsdale, USA}
}

@inproceedings{Scheibler2018PyRoom,
	year = 2018,
	month = apr,
	author = {Robin Scheibler and Eric Bezzam and Ivan Dokmanic},
	title = {Pyroomacoustics: A Python Package for Audio Room Simulation and Array Processing Algorithms},
	booktitle=ICASSP,
    address = {Calgary, Canada}
}

@article{kingma2015adam,
  author={Diederik P. Kingma and Jimmy Ba},
  title={Adam: A Method for Stochastic Optimization},
  journal=ICLR,
  year={2015}
}

@book{sarkka2019sde,
  title = {Applied Stochastic Differential Equations},
  author = {Särkkä, Simo and Solin, Arno},
  year = {2019},
  publisher = {{Cambridge University Press}},
  location = {{Cambridge ; New York, NY}},
}

@article{Fu2022MetricGAN+,
  title={{MetricGAN-U}: Unsupervised speech enhancement/dereverberation based only on noisy/reverberated speech},
  author={Fu, Szu-Wei and Yu, Cheng and Hung, Kuo-Hsuan and Ravanelli, Mirco and Tsao, Yu},
  journal=ICASSP,
  pages={7412--7416},
  year={2022},
}

@inproceedings{Liu2022NeuralVI,
  title={Neural Vocoder is All You Need for Speech Super-resolution},
  author={Haohe Liu and Woo Yong Choi and Xubo Liu and Qiuqiang Kong and Qiao Tian and Deliang Wang},
  booktitle=INTERSPEECH,
  year={2022},
  address={Incheon, South Korea},
  month=sep
}

@inproceedings{Lee2021NUWaveAD,
  title={{NU}-Wave: A Diffusion Probabilistic Model for Neural Audio Upsampling},
  author={Junhyeok Lee and Seungu Han},
  booktitle=Interspeech,
  year={2021},
  month=sep,
  address = {Brno, Czech Republic}
}

@inproceedings{Leroux2019SISDR,
  author = {Roux, Jonathan Le and Wisdom, Scott and Erdogan, Hakan and Hershey, John R.},
  title = {{SDR} - {H}alf-baked or well done?},
  year = {2019},
  booktitle=ICASSP,
  address = {Brighton, UK},
  month = may
 }
 
 @INPROCEEDINGS{Rix2001PESQ,  
 author={Rix, A.W. and Beerends, J.G. and Hollier, M.P. and Hekstra, A.P.},  
 booktitle=ICASSP, 
 title={Perceptual evaluation of speech quality ({PESQ})-a new method for speech quality assessment of telephone networks and codecs},   
 year={2001},
 month = may,
 address = {Salt Lake City, USA}
 }
 
 @inproceedings{Kong2020HiFiGAN,
  author = {Kong, Jungil and Kim, Jaehyeon and Bae, Jaekyoung},
  title = {HiFi-GAN: Generative Adversarial Networks for Efficient and High Fidelity Speech Synthesis},
  year = {2020},
  booktitle=NIPS
}

@inproceedings{Han2022NUWave2,
  title={NU-Wave 2: A General Neural Audio Upsampling Model for Various Sampling Rates},
  author={Han, Seungu and Lee, Junhyeok},
  booktitle=Interspeech,
  year={2022},
  month=sep,
  address={Singapore, Singapore}
}

@article{Thaal2011STOI,  author={Taal, Cees H. and Hendriks, Richard C. and Heusdens, Richard and Jensen, Jesper},  journal=TASLIEEE,   title={An Algorithm for Intelligibility Prediction of Time–Frequency Weighted Noisy Speech},   year={2011},
  volume={19},
  number={7},
  pages={2125-2136}
}


@book{MurphyBook2,
 author = {Kevin P. Murphy},
 title = {Probabilistic Machine Learning: Advanced Topics},
 publisher = {MIT Press},
 year = 2023
}

@article{Lemercier2022storm,
  author = {Lemercier, Jean-Marie and Richter, Julius and Welker, Simon and Gerkmann, Timo},
  title = {{S}to{RM}: A Diffusion-based Stochastic Regeneration Model for Speech Enhancement and Dereverberation},
  journal = {arXiv},
  year = {2022}
}

